Contributions to Khovanov Homology

Khovanov homology ist a new link invariant, discovered by M. Khovanov, and used by J. Rasmussen to give a combinatorial proof of the Milnor conjecture. In this thesis, we give examples of mutant links with different Khovanov homology. We prove that Khovanov's chain complex retracts to a subcomplex, whose generators are related to spanning trees of the Tait graph, and we exploit this result to investigate the structure of Khovanov homology for alternating knots. Further, we extend Rasmussen's invariant to links. Finally, we generalize Khovanov's categorifications of the colored Jones polynomial, and study conditions under which our categorifications are functorial with respect to colored framed link cobordisms. In this context, we develop a theory of Carter--Saito movie moves for framed link cobordisms.

==> kinocontab.tex <==
%\advance\hsize 1.4truein \advance\hoffset -0.7truein
%\advance\vsize 1.0truein \advance\voffset -0.5truein

\def\Cal#1{{\fam2#1}}

\let\TSp\thinspace
\let\NSp\negthinspace
\def\DSp{\thinspace\thinspace}
\def\QSp{\thinspace\thinspace\thinspace\thinspace}

%\nopagenumbers
\offinterlineskip

\def\gobble#1{}
\def\hline{\noalign{\hrule}}
\def\dblhline{height 0.16667em\gobble&&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
&\vrule&
\cr
\noalign{\hrule}}

\def\group#1#2#3#4{${\raise 1pt%
\hbox{#4#1\ifnum#2=0\else[#2]\fi}\over\lower 3pt\hbox{#4#3}}$}
\def\putdown#1{\smash{\vtop{\null\hbox{#1}}}}

\null\vfill
$$\vbox{\ialign{%
\vrule\TSp\vrule #\strut&\DSp\hfil #\DSp\vrule\TSp\vrule&\kern.75em
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp&\hfil #\hfil&
\TSp\hfil #\hfil\TSp\kern.75em\vrule\TSp\vrule\cr
%
\hline\dblhline
height 11pt depth 4pt&&
-7&\vrule&
-6&\vrule&
-5&\vrule&
-4&\vrule&
-3&\vrule&
-2&\vrule&
-1&\vrule&
0&\vrule&
1&\vrule&
2&\vrule&
3&\vrule&
4&\vrule&
5&\vrule&
6\cr\hline\dblhline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&&
&&
&&
&&
&&
&&
&&
&\QSp\putdown{1}\QSp&
&\QSp\putdown{5}\QSp&
&\DSp\putdown{10}\DSp&
&\DSp\putdown{10}\DSp&
&\QSp\putdown{6}\QSp&
&\QSp\putdown{1}\QSp&\cr
&9&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\group{0}{0}{1}{}&\rightarrowfill&
\group{0}{0}{6}{}&\rightarrowfill&
\group{0}{0}{15}{}&\rightarrowfill&
\group{0}{0}{20}{}&\rightarrowfill&
\group{0}{0}{16}{}&\rightarrowfill&
\group{1}{0}{8}{\bf}&\rightarrowfill&
\group{0}{0}{1}{}\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&&
&&
&&
&&
&&
&\QSp\putdown{1}\QSp&
&\DSp\putdown{12}\DSp&
&\DSp\putdown{55}\DSp&
&\TSp\putdown{125}\TSp&
&\TSp\putdown{154}\TSp&
&\TSp\putdown{107}\TSp&
&\DSp\putdown{41}\DSp&
&\QSp\putdown{4}\QSp&\cr
&7&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\group{0}{0}{1}{}&\rightarrowfill&
\group{0}{0}{13}{}&\rightarrowfill&
\group{0}{0}{67}{}&\rightarrowfill&
\group{0}{0}{180}{}&\rightarrowfill&
\group{0}{0}{279}{}&\rightarrowfill&
\group{0}{0}{261}{}&\rightarrowfill&
\group{1}{0}{149}{\bf}&\rightarrowfill&
\group{0}{1}{45}{\bf}&\rightarrowfill&
\group{0}{0}{4}{}\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&&
&&
&&
&&
&\QSp\putdown{5}\QSp&
&\DSp\putdown{55}\DSp&
&\TSp\putdown{260}\TSp&
&\TSp\putdown{658}\TSp&
&\TSp\putdown{951}\TSp&
&\TSp\putdown{792}\TSp&
&\TSp\putdown{371}\TSp&
&\DSp\putdown{89}\DSp&
&\QSp\putdown{6}\QSp&\cr
&5&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\group{0}{0}{5}{}&\rightarrowfill&
\group{0}{0}{60}{}&\rightarrowfill&
\group{0}{0}{315}{}&\rightarrowfill&
\group{0}{0}{918}{}&\rightarrowfill&
\group{0}{0}{1609}{}&\rightarrowfill&
\group{0}{0}{1743}{}&\rightarrowfill&
\group{1}{0}{1164}{\bf}&\rightarrowfill&
\group{1}{1}{461}{\bf}&\rightarrowfill&
\group{0}{0}{95}{}&\rightarrowfill&
\group{0}{0}{6}{}\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&&
&&
&&
&\DSp\putdown{10}\DSp&
&\TSp\putdown{126}\TSp&
&\TSp\putdown{663}\TSp&
&\TSp\putdown{1895}\TSp&
&\TSp\putdown{3159}\TSp&
&\TSp\putdown{3104}\TSp&
&\TSp\putdown{1767}\TSp&
&\TSp\putdown{565}\TSp&
&\DSp\putdown{91}\DSp&
&\QSp\putdown{4}\QSp&\cr
&3&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\group{0}{0}{10}{}&\rightarrowfill&
\group{0}{0}{136}{}&\rightarrowfill&
\group{0}{0}{789}{}&\rightarrowfill&
\group{0}{0}{2558}{}&\rightarrowfill&
\group{0}{0}{5054}{}&\rightarrowfill&
\group{1}{0}{6264}{\bf}&\rightarrowfill&
\group{2}{0}{4873}{\bf}&\rightarrowfill&
\group{1}{1}{2333}{\bf}&\rightarrowfill&
\group{0}{0}{656}{}&\rightarrowfill&
\group{0}{0}{95}{}&\rightarrowfill&
\group{0}{0}{4}{}\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&&
&&
&\DSp\putdown{10}\DSp&
&\TSp\putdown{158}\TSp&
&\TSp\putdown{983}\TSp&
&\TSp\putdown{3241}\TSp&
&\TSp\putdown{6238}\TSp&
&\TSp\putdown{7166}\TSp&
&\TSp\putdown{4871}\TSp&
&\TSp\putdown{1916}\TSp&
&\TSp\putdown{417}\TSp&
&\DSp\putdown{44}\DSp&
&\QSp\putdown{1}\QSp&\cr
&1&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\group{0}{0}{10}{}&\rightarrowfill&
\group{0}{0}{168}{}&\rightarrowfill&
\group{0}{0}{1141}{}&\rightarrowfill&
\group{0}{0}{4224}{}&\rightarrowfill&
\group{0}{0}{9479}{}&\rightarrowfill&
\group{2}{0}{13406}{\bf}&\rightarrowfill&
\group{1}{1}{12038}{\bf}&\rightarrowfill&
\group{1}{2}{6788}{\bf}&\rightarrowfill&
\group{0}{0}{2333}{}&\rightarrowfill&
\group{0}{0}{461}{}&\rightarrowfill&
\group{0}{0}{45}{}&\rightarrowfill&
\group{0}{0}{1}{}\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&&
&\QSp\putdown{6}\QSp&
&\TSp\putdown{113}\TSp&
&\TSp\putdown{859}\TSp&
&\TSp\putdown{3375}\TSp&
&\TSp\putdown{7607}\TSp&
&\TSp\putdown{10219}\TSp&
&\TSp\putdown{8186}\TSp&
&\TSp\putdown{3850}\TSp&
&\TSp\putdown{1023}\TSp&
&\TSp\putdown{141}\TSp&
&\QSp\putdown{8}\QSp&
&&\cr
&-1&
&\smash{\vrule height 15pt}&
\group{0}{0}{6}{}&\rightarrowfill&
\group{0}{0}{119}{}&\rightarrowfill&
\group{0}{0}{972}{}&\rightarrowfill&
\group{0}{0}{4234}{}&\rightarrowfill&
\group{0}{0}{10982}{}&\rightarrowfill&
\group{1}{0}{17827}{\bf}&\rightarrowfill&
\group{3}{1}{18408}{\bf}&\rightarrowfill&
\group{2}{1}{12038}{\bf}&\rightarrowfill&
\group{0}{0}{4873}{}&\rightarrowfill&
\group{0}{0}{1164}{}&\rightarrowfill&
\group{0}{0}{149}{}&\rightarrowfill&
\group{0}{0}{8}{}&\smash{\vrule height 15pt}&
\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&\QSp\putdown{1}\QSp&
&\DSp\putdown{42}\DSp&
&\TSp\putdown{432}\TSp&
&\TSp\putdown{2128}\TSp&
&\TSp\putdown{5788}\TSp&
&\TSp\putdown{9186}\TSp&
&\TSp\putdown{8639}\TSp&
&\TSp\putdown{4766}\TSp&
&\TSp\putdown{1498}\TSp&
&\TSp\putdown{245}\TSp&
&\DSp\putdown{16}\DSp&
&&
&&\cr
&-3&
\group{0}{0}{1}{}&\rightarrowfill&
\group{0}{0}{43}{}&\rightarrowfill&
\group{0}{0}{474}{}&\rightarrowfill&
\group{0}{0}{2560}{}&\rightarrowfill&
\group{0}{0}{7916}{}&\rightarrowfill&
\group{2}{0}{14976}{\bf}&\rightarrowfill&
\group{2}{1}{17827}{\bf}&\rightarrowfill&
\group{1}{1}{13406}{\bf}&\rightarrowfill&
\group{0}{0}{6264}{}&\rightarrowfill&
\group{0}{0}{1743}{}&\rightarrowfill&
\group{0}{0}{261}{}&\rightarrowfill&
\group{0}{0}{16}{}&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&\QSp\putdown{5}\QSp&
&\TSp\putdown{113}\TSp&
&\TSp\putdown{784}\TSp&
&\TSp\putdown{2708}\TSp&
&\TSp\putdown{5207}\TSp&
&\TSp\putdown{5774}\TSp&
&\TSp\putdown{3704}\TSp&
&\TSp\putdown{1350}\TSp&
&\TSp\putdown{259}\TSp&
&\DSp\putdown{20}\DSp&
&&
&&
&&\cr
&-5&
\group{0}{0}{5}{}&\rightarrowfill&
\group{0}{0}{118}{}&\rightarrowfill&
\group{0}{0}{897}{}&\rightarrowfill&
\group{0}{0}{3492}{}&\rightarrowfill&
\group{1}{0}{7916}{\bf}&\rightarrowfill&
\group{1}{2}{10982}{\bf}&\rightarrowfill&
\group{1}{1}{9479}{\bf}&\rightarrowfill&
\group{0}{0}{5054}{}&\rightarrowfill&
\group{0}{0}{1609}{}&\rightarrowfill&
\group{0}{0}{279}{}&\rightarrowfill&
\group{0}{0}{20}{}&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&\DSp\putdown{10}\DSp&
&\TSp\putdown{152}\TSp&
&\TSp\putdown{745}\TSp&
&\TSp\putdown{1814}\TSp&
&\TSp\putdown{2418}\TSp&
&\TSp\putdown{1805}\TSp&
&\TSp\putdown{753}\TSp&
&\TSp\putdown{165}\TSp&
&\DSp\putdown{15}\DSp&
&&
&&
&&
&&\cr
&-7&
\group{0}{0}{10}{}&\rightarrowfill&
\group{0}{0}{162}{}&\rightarrowfill&
\group{0}{0}{897}{}&\rightarrowfill&
\group{1}{0}{2560}{\bf}&\rightarrowfill&
\group{2}{1}{4234}{\bf}&\rightarrowfill&
\group{1}{0}{4224}{\bf}&\rightarrowfill&
\group{0}{0}{2558}{}&\rightarrowfill&
\group{0}{0}{918}{}&\rightarrowfill&
\group{0}{0}{180}{}&\rightarrowfill&
\group{0}{0}{15}{}&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&\DSp\putdown{10}\DSp&
&\TSp\putdown{108}\TSp&
&\TSp\putdown{365}\TSp&
&\TSp\putdown{606}\TSp&
&\TSp\putdown{535}\TSp&
&\TSp\putdown{254}\TSp&
&\DSp\putdown{61}\DSp&
&\QSp\putdown{6}\QSp&
&&
&&
&&
&&
&&\cr
&-9&
\group{0}{0}{10}{}&\rightarrowfill&
\group{0}{0}{118}{}&\rightarrowfill&
\group{1}{0}{474}{\bf}&\rightarrowfill&
\group{1}{1}{972}{\bf}&\rightarrowfill&
\group{0}{0}{1141}{}&\rightarrowfill&
\group{0}{0}{789}{}&\rightarrowfill&
\group{0}{0}{315}{}&\rightarrowfill&
\group{0}{0}{67}{}&\rightarrowfill&
\group{0}{0}{6}{}&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&\QSp\putdown{5}\QSp&
&\DSp\putdown{38}\DSp&
&\DSp\putdown{80}\DSp&
&\DSp\putdown{88}\DSp&
&\DSp\putdown{48}\DSp&
&\DSp\putdown{12}\DSp&
&\QSp\putdown{1}\QSp&
&&
&&
&&
&&
&&
&&\cr
&-11&
\group{0}{0}{5}{}&\rightarrowfill&
\group{0}{0}{43}{}&\rightarrowfill&
\group{1}{1}{119}{\bf}&\rightarrowfill&
\group{0}{0}{168}{}&\rightarrowfill&
\group{0}{0}{136}{}&\rightarrowfill&
\group{0}{0}{60}{}&\rightarrowfill&
\group{0}{0}{13}{}&\rightarrowfill&
\group{0}{0}{1}{}&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
height 0.2em depth 0.2em\gobble&&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
&\vrule depth0pt&
\cr
height 0pt\gobble&&
&\QSp\putdown{1}\QSp&
&\QSp\putdown{4}\QSp&
&\QSp\putdown{6}\QSp&
&\QSp\putdown{4}\QSp&
&\QSp\putdown{1}\QSp&
&&
&&
&&
&&
&&
&&
&&
&&\cr
&-13&
\group{0}{0}{1}{}&\rightarrowfill&
\group{1}{0}{6}{\bf}&\rightarrowfill&
\group{0}{0}{10}{}&\rightarrowfill&
\group{0}{0}{10}{}&\rightarrowfill&
\group{0}{0}{5}{}&\rightarrowfill&
\group{0}{0}{1}{}&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
&\smash{\vrule height 15pt}&
\cr
height 0.3em\gobble&&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
&\smash{\vrule height 10pt}&
\cr
\hline
%
\dblhline
}}$$

%\medskip\centerline{Dimensions of $\Cal{H}^{i,j}$ and
%$\Cal{C}^{i,j}$ and ranks of chain differentials}
%\medskip
%\centerline{for the Kinoshita-Terasaka knot}
%\vfill
%\bye

